Deep Reinforcement Learning with Shallow Controllers: An Experimental Application to PID Tuning

Deep reinforcement learning (RL) is an optimization-driven framework for producing control strategies for general dynamical systems without explicit reliance on process models. Good results have been reported in simulation. Here we demonstrate the challenges in implementing a state of the art deep RL algorithm on a real physical system. Aspects include the interplay between software and existing hardware; experiment design and sample efficiency; training subject to input constraints; and interpretability of the algorithm and control law. At the core of our approach is the use of a PID controller as the trainable RL policy. In addition to its simplicity, this approach has several appealing features: No additional hardware needs to be added to the control system, since a PID controller can easily be implemented through a standard programmable logic controller; the control law can easily be initialized in a "safe'' region of the parameter space; and the final product -- a well-tuned PID controller -- has a form that practitioners can reason about and deploy with confidence.

==> arXiv v1/figures/table_RLexperimentSpecs.tex <==
\resizebox{\linewidth}{!}{%
\begin{tabular}{ l *{16}{c} }
\toprule
\hspace*{2cm} &
\multicolumn{7}{c}{RL (Unconstrained)} &
\multicolumn{3}{c}{RL (Constrained)} & \multicolumn{5}{c}{SIMC} & \multicolumn{1}{c}{Accutune}\\
\cmidrule(lr){2-8} \cmidrule(lr){9-11} \cmidrule(lr){12-16} \cmidrule(lr){17-17}
&
\makebox[1em]{1} &
\textbf{\makebox[1em]{2}} &
\textbf{\makebox[1em]{3}} &
\makebox[1em]{4} &
\makebox[1em]{5} &
\makebox[1em]{6} &
\makebox[1em]{7} &
\textbf{\makebox[1em]{8}} &
\makebox[1em]{9} &
\makebox[1em]{10} &
\makebox[1em]{1} &
\makebox[1em]{2} &
\textbf{\makebox[1em]{3}} &
\makebox[1em]{4} &
\makebox[1em]{5} &
\textbf{\makebox[1em]{1}} \\
\midrule
Reward & Eq. \eqref{eq:baselineReward1} & \eqref{eq:baselineReward2} & \eqref{eq:baselineReward2} & \eqref{eq:baselineReward1} & \eqref{eq:hybridPenalty} & \eqref{eq:hybridReward} & \eqref{eq:hybridReward} & \eqref{eq:baselineReward2} & \eqref{eq:hybridReward} & \eqref{eq:hybridReward} 	& - & - & - & - & - & - 			\\
Initialization & $k_p=$ 4.0 & 4.0 & 2.0 & 2.0 & 4.0 & 4.0 & 2.0 & 4.0 & 4.0 & 4.0 	& - & - & - & - & - & - 				\\
Setting & - & - & - & - & - & - & - & - & - & - & $T_c=$ 9.21 & 15 & 20 & 25 & 30 & 	Mode=``slow"\\
%Misc. & x & x & x & x & x & x & x & x & x \\
\bottomrule
\end{tabular}
}

==> arXiv v1/figures/table_Robustness_allExperiments.tex <==
\resizebox{\linewidth}{!}{%
\begin{tabular}{NPPPPPPc}
\toprule
\multicolumn{0}{l}{}  &              \multicolumn{2}{r}{IAE} &              \multicolumn{2}{c}{ISE} &            \multicolumn{2}{c}{TV} &          \multicolumn{2}{c}{TV$_u$} &          \multicolumn{2}{c}{$\%$ OS} &                \multicolumn{2}{c}{ST} & $\text{M}_s$ \\
\midrule
RL-\therowcntr\label{row:robustness_td3_2021_04_07_1103}   &   44.41&9.57 &   28.33&4.89 &  1.88&0.23 &  11.14&1.08 &  22.94&10.77 &  134.67&25.51 & 1.55\\
\textbf{RL-\therowcntr}\label{row:robustness_td3_2021_04_07_1208}   &   43.76&7.59 &   30.18&3.85 &  1.56&0.12 &   9.63&0.50 &   10.95&8.26 &  129.08&34.22 & 1.35\\
\textbf{RL-\therowcntr}\label{row:robustness_td3_2021_04_07_1357}   &   48.75&4.55 &   34.00&3.40 &  1.42&0.05 &   8.90&0.20 &    7.46&2.03 &  153.17&26.34 & 1.25\\
RL-\therowcntr\label{row:robustness_td3_2021_04_07_1518}   &  67.96&15.42 &  40.09&10.96 &  2.32&0.40 &  12.81&1.92 &  48.20&14.38 &  186.58&28.46 & 1.42\\
RL-\therowcntr\label{row:robustness_td3_2021_04_29_1040}   &   42.72&8.03 &   27.87&4.16 &  1.78&0.21 &  10.67&0.91 &   20.43&9.74 &  128.75&15.36 & 1.48\\
RL-\therowcntr\label{row:robustness_td3_2021_04_29_1133}   &   40.85&7.63 &   27.00&3.81 &  1.69&0.23 &  10.32&1.14 &   17.33&9.84 &  145.42&41.48 & 1.50\\
RL-\therowcntr\label{row:robustness_td3_2021_04_30_1426}       &   54.92&6.65 &   34.65&2.94 &  1.50&0.09 &      9.06&0.47 &   14.87&4.67 &  190.58&34.84 & 1.27\\
\textbf{RL-\therowcntr}\label{row:robustness_td3_2021_04_28_1451}   &   42.75&5.87 &   28.89&3.75 &  1.56&0.09 &   9.62&0.41 &   11.38&6.48 &  166.42&20.03 & 1.36\\
RL-\therowcntr\label{row:robustness_td3_2021_05_14_1127}   &  56.47&13.25 &   33.90&7.48 &  2.06&0.25 &  11.45&1.25 &   37.84&9.84 &  163.08&21.80 & 1.51\\
RL-\therowcntr\label{row:robustness_td3_2021_07_12_1047}\setcounter{rowcntr}{0}  &   40.18&6.59 &   27.84&3.61 &  1.58&0.13 &   9.81&0.52 &   11.08&7.57 &   133.17&5.63 & 1.41\\
SIMC-\therowcntr\label{row:robustness_SIMC9} &  61.64&17.36 &  36.73&10.19 &  2.68&0.72 &  14.29&3.40 &  53.55&14.48 &  162.08&52.19 & 1.72\\
SIMC-\therowcntr\label{row:robustness_SIMC15} &  56.16&10.89 &   34.36&6.05 &  1.73&0.11 &  10.07&0.49 &   24.11&7.83 &  168.17&29.17 & 1.36\\
\textbf{SIMC-\therowcntr}\label{row:robustness_SIMC20} &   54.74&6.49 &   35.47&3.20 &  1.52&0.02 &   9.17&0.05 &   13.26&4.97 &  193.75&19.16 & 1.25\\
SIMC-\therowcntr\label{row:robustness_SIMC25} &   57.61&5.08 &   39.12&3.50 &  1.38&0.02 &   8.49&0.11 &    8.38&2.57 &  167.17&47.65 & 1.19\\
SIMC-\therowcntr\label{row:robustness_SIMC30}\setcounter{rowcntr}{0} &  57.33&12.18 &   38.77&9.85 &  1.33&0.06 &   8.31&0.34 &    4.86&1.79 &  141.67&13.73 & 1.16\\
\textbf{Accutune-\therowcntr}\label{row:robustness_AccuSlow}  &  70.09&24.46 &  46.33&16.94 &  1.59&0.24 &  351.62&201.09 &    8.98&0.46 &  139.33&65.07 & 1.41\\
\bottomrule
\end{tabular}
}

% See https://tex.stackexchange.com/questions/305395/table-alignment-around-pm-sign-how-to-have-good-alignment-without-pm-where-a

%
%\resizebox{\linewidth}{!}{%
%\begin{tabular}{ND{,}{\pm}{-1}D{,}{\pm}{-1}D{,}{\pm}{-1}D{,}{\pm}{-1}D{,}{\pm}{-1}D{,}{\pm}{-1}}
%\toprule
%\multicolumn{0}{l}{}  &              \multicolumn{1}{r}{IAE} &              \multicolumn{1}{c}{ISE} &            \multicolumn{1}{c}{TV} &          \multicolumn{1}{c}{TV$_u$} &          \multicolumn{1}{c}{$\%$ OS} &                \multicolumn{1}{c}{ST} \\
%\midrule
%RL-\therowcntr\label{row:robustness_td3_2021_04_07_1103}   &   44.41,9.57 &   28.33,4.89 &  1.88,0.23 &  11.14,1.08 &  22.94,10.77 &  134.67,25.51 \\
%RL-\therowcntr\label{row:robustness_td3_2021_04_07_1208}   &   43.76,7.59 &   30.18,3.85 &  1.56,0.12 &   9.63,0.50 &   10.95,8.26 &  129.08,34.22 \\
%RL-\therowcntr\label{row:robustness_td3_2021_04_07_1357}   &   48.75,4.55 &   34.00,3.40 &  1.42,0.05 &   8.90,0.20 &    7.46,2.03 &  153.17,26.34 \\
%RL-\therowcntr\label{row:robustness_td3_2021_04_07_1518}   &  67.96,15.42 &  40.09,10.96 &  2.32,0.40 &  12.81,1.92 &  48.20,14.38 &  186.58,28.46 \\
%RL-\therowcntr\label{row:robustness_td3_2021_04_29_1040}   &   42.72,8.03 &   27.87,4.16 &  1.78,0.21 &  10.67,0.91 &   20.43,9.74 &  128.75,15.36 \\
%RL-\therowcntr\label{row:robustness_td3_2021_04_29_1133}   &   40.85,7.63 &   27.00,3.81 &  1.69,0.23 &  10.32,1.14 &   17.33,9.84 &  145.42,41.48 \\
%RL-\therowcntr\label{row:robustness_td3_2021_04_30_1426}       &   54.92,6.65 &   34.65,2.94 &  1.50,0.09 &      9.06,0.47 &   14.87,4.67 &  190.58,34.84 \\
%RL-\therowcntr\label{row:robustness_td3_2021_04_28_1451}   &   42.75,5.87 &   28.89,3.75 &  1.56,0.09 &   9.62,0.41 &   11.38,6.48 &  166.42,20.03 \\
%RL-\therowcntr\label{row:robustness_td3_2021_05_14_1127}   &  56.47,13.25 &   33.90,7.48 &  2.06,0.25 &  11.45,1.25 &   37.84,9.84 &  163.08,21.80 \\
%RL-\therowcntr\label{row:robustness_td3_2021_07_12_1047}\setcounter{rowcntr}{0}  &   40.18,6.59 &   27.84,3.61 &  1.58,0.13 &   9.81,0.52 &   11.08,7.57 &   133.17,5.63 \\
%SIMC-\therowcntr\label{row:robustness_SIMC9} &  61.64,17.36 &  36.73,10.19 &  2.68,0.72 &  14.29,3.40 &  53.55,14.48 &  162.08,52.19 \\
%SIMC-\therowcntr\label{row:robustness_SIMC15} &  56.16,10.89 &   34.36,6.05 &  1.73,0.11 &  10.07,0.49 &   24.11,7.83 &  168.17,29.17 \\
%SIMC-\therowcntr\label{row:robustness_SIMC20} &   54.74,6.49 &   35.47,3.20 &  1.52,0.02 &   9.17,0.05 &   13.26,4.97 &  193.75,19.16 \\
%SIMC-\therowcntr\label{row:robustness_SIMC25} &   57.61,5.08 &   39.12,3.50 &  1.38,0.02 &   8.49,0.11 &    8.38,2.57 &  167.17,47.65 \\
%SIMC-\therowcntr\label{row:robustness_SIMC30}\setcounter{rowcntr}{0} &  57.33,12.18 &   38.77,9.85 &  1.33,0.06 &   8.31,0.34 &    4.86,1.79 &  141.67,13.73 \\
%Accutune--\therowcntr\label{row:robustness_AccuSlow}  &  70.09,24.46 &  46.33,16.94 &  1.59,0.24 &  351.62,201.09 &    8.98,0.46 &  139.33,65.07 \\
%\bottomrule
%\end{tabular}
%}


==> arXiv v1/figures/table_hyperparameters.tex <==
\resizebox{\textwidth}{!}{%
\begin{tabular}{l* {2}{c}}
\toprule
Hyperparameter &    Symbol &    Nominal value\\
\midrule
Actor learning rate & $\alpha_c$ & $0.002$ \\
Critic learning rate & $\alpha_c$ & $0.002$ \\
Discount factor & $\gamma$ & $0.99$ \\
Target network update rate & $\rho$ & $0.995$ \\
Policy update delay &  \texttt{policy\_{delay}} & $2$ \\
Batch size & $\abs{\mathcal{B}}$ & $256$ \\
Replay buffer size & $\abs{\mathcal{D}_{\text{RM}}}$ & $10,000$ \\
Target noise & $\sigma$ & $0.2$ \\
\bottomrule
\end{tabular}
}
% see https://tex.stackexchange.com/questions/356815/reference-table-row-in-latex
% see https://www.overleaf.com/learn/latex/Counters#Reference_guide
% Use the following in the preamble
    % \newcounter{rowcntr}[table]
    % \renewcommand{\therowcntr}{\arabic{rowcntr}}
    % % A new columntype to apply automatic stepping
    % \newcolumntype{N}{>{\refstepcounter{rowcntr}}l}
    % % Reset the rowcntr counter at each new tabular
    % \AtBeginEnvironment{tabular}{\setcounter{rowcntr}{0}}
    % \newcommand{\rowref}[2]{#1-\ref*{#2}}
% The idea is to allocate a a custom column for labels and indices that can then be references in the text
% We also define a command \rowref so the acronyms can be incorporated when referencing a row




==> arXiv v1/figures/table_scorecard.tex <==
\begin{tabularx}{0.80\linewidth}{lYYYYYYY} %l|X|X|X|X|X|X|X|X|
% \toprule
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\rot{Nominal performance}} & \multicolumn{1}{c}{\rot{Robustness}} & \multicolumn{1}{c}{\rot{Time required for tuning}} & \multicolumn{1}{c}{\rot{Disturbance to process}} & \multicolumn{1}{c}{\rot{Hardware requirements}} & \multicolumn{1}{c}{\rot{Ease of use}} & \multicolumn{1}{c}{\rot{Input constraints}}\\
% \cline{2-9}
\midrule
% \cline{2-9}
SIMC & -- & -- & -- & \xmark & \cmark & -- & \xmark \\
% \cline{2-9}
Accutune III & \xmark & \xmark & \cmark & \cmark & \cmark & \cmark & \xmark \\
% \cline{2-9}
Deep RL & \cmark & \cmark & \xmark & \cmark & -- & \cmark  & \cmark \\
% \cline{2-9}
\bottomrule
\end{tabularx}


==> arXiv v1/figures/table_subsetExperiments_nominal.tex <==
\resizebox{\linewidth}{!}{%
\begin{tabular}{Nlllllll}
\toprule
\multicolumn{0}{l}{} &    IAE &    ISE &    TV & TV$_u$ & $\%$ OS &      ST & $\text{M}_s$ \\
\midrule
RL\label{row:nominal_RL}   &  $39.34\pm3.44$ &  $27.56\pm2.25$ &  $1.49\pm0.08$ &   \phantom{00}$9.37\pm0.42$ &    $6.39\pm1.21$ &   $127.00\pm38.80$ & $1.32\pm0.06$ \\
SIMC\label{row:nominal_SIMC20} &  47.74 &  32.31 &  1.50 &   \phantom{00}9.14 &    7.81 &  215.25 & 1.25\\
Accutune\label{row:nominal_AccuSlow} &  54.06 &  34.06 &  1.75 &  583.78 &    9.14 &  159.75 & 1.41\\
\bottomrule
\end{tabular}
}
% see https://tex.stackexchange.com/questions/356815/reference-table-row-in-latex
% see https://www.overleaf.com/learn/latex/Counters#Reference_guide
% Use the following in the preamble
    % \newcounter{rowcntr}[table]
    % \renewcommand{\therowcntr}{\arabic{rowcntr}}
    % % A new columntype to apply automatic stepping
    % \newcolumntype{N}{>{\refstepcounter{rowcntr}}l}
    % % Reset the rowcntr counter at each new tabular
    % \AtBeginEnvironment{tabular}{\setcounter{rowcntr}{0}}
    % \newcommand{\rowref}[2]{#1-\ref*{#2}}
% The idea is to allocate a a custom column for labels and indices that can then be references in the text
% We also define a command \rowref so the acronyms can be incorporated when referencing a row so the acronyms can be incorporated when referencing a row

